Exploring the string shoving model in PYTHIA8 for collective behaviors in $pp$ collisions

Two-particle correlations have been used to study property of a produced medium called Quark-Gluon Plasma (QGP) in relativistic heavy-ion collisions, and a long-range correlation among produced particles has been considered as a strong evidence of strongly interacting QGP. Strikingly, clear long-range correlations have been also observed in small collision systems like $pp$ and $p$+$A$ at a wide range of collision energies. A model introducing a repulsive force between flux tubes called string shoving can qualitatively describe the long-range near-side correlations in high multiplicity $pp$ collisions. This model implemented in the PYTHIA Monte Carlo event generator allows us to perform detailed study. In this work, a full data analysis to calculate associated yields and flow coefficients is performed with PYTHIA events, and the results are compared with experimental results. We find that the string shoving model overestimates long-range near-side correlations particularly in low multiplicity events. We also introduce a method to subtract such overestimated correlations in low multiplicity to have a more relevant comparison with the data.

==> commands.tex <==
% $Id: commands.tex 934 2013-06-19 20:56:45Z mfloris $

\newcommand{\pp}{\mbox{$pp$}\xspace}
\newcommand{\pythia}{\textsc{Pythia8}\xspace}
\newcommand{\deta}{\mbox{$\Delta\eta$}\xspace}
\newcommand{\pt}{\mbox{$p_{T}$}\xspace}
\newcommand{\pT}{\mbox{$p_{T}$}\xspace}

\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\mrmo}[1]{\mathrm{\overline{#1}}}
\newcommand{\bsb}[1]{\boldsymbol{#1}}
\newcommand{\circit}{\item[$\circ$]}

\newcommand{\ITS}          {\rm{ITS}}
\newcommand{\TOF}          {\rm{TOF}}
\newcommand{\ZDC}          {\rm{ZDC}}
\newcommand{\ZDCs}         {\rm{ZDCs}}
\newcommand{\ZNA}          {\rm{ZNA}}
\newcommand{\ZNC}          {\rm{ZNC}}
\newcommand{\SPD}          {\rm{SPD}}
\newcommand{\SDD}          {\rm{SDD}}
\newcommand{\SSD}          {\rm{SSD}}
\newcommand{\TPC}          {\rm{TPC}}
\newcommand{\VZERO}        {\rm{VZERO}}
\newcommand{\VZEROA}       {\rm{VZERO-A}}
\newcommand{\VZEROC}       {\rm{VZERO-C}}
\newcommand{\pip}          {$\pi^{+}$}
\newcommand{\pim}          {$\pi^{-}$}
\newcommand{\kap}          {K$^{+}$}
\newcommand{\kam}          {K$^{-}$}
\newcommand{\pbar}         {$\rm\overline{p}$}
\newcommand{\kzero}        {\ensuremath{{\rm K}^{0}_{S}}}
\newcommand{\kstar}        {\ensuremath{{\rm K}^{*}}}
\newcommand{\He}           {\ensuremath{^{3}{\rm He}}}
\newcommand{\LH}           {\ensuremath{^{3}_{\Lambda}{\rm H}}}
\newcommand{\vzero}        {\ensuremath{{\rm V}^0}}
\newcommand{\lmb}          {\ensuremath{\Lambda}}
\newcommand{\almb}         {\ensuremath{\bar{\Lambda}}}
\newcommand{\allpart}      {$\pi^{\pm}$, K$^{\pm}$, \kzero, p(\pbar) and \lmb(\almb)}
\newcommand{\allpi}        {$\pi^{\pm}$}
\newcommand{\allk}         {K$^{\pm}$}
\newcommand{\allp}         {p(\pbar)}
\newcommand{\alllmb}       {\lmb(\almb)}
\newcommand{\degree}       {$^{\rm o}$}
\newcommand{\dg}           {\mbox{$^\circ$}}
\newcommand{\dedx}         {\ensuremath{\mathrm{d}E/\mathrm{d}x}}
\newcommand{\dndy}         {d$N$/d$y$}
\newcommand {\ee}            {\mbox{e$^+$e$^-$}}
%\newcommand{\pp}           {pp}
\newcommand{\ppbar}        {\mbox{$\mathrm {p\overline{p}}$}}
\newcommand{\PbPb}         {\mbox{Pb--Pb}}
\newcommand{\pPb}          {\mbox{p--Pb}}
\newcommand{\AuAu}         {\mbox{Au--Au}}
\newcommand{\pseudorap}    {\mbox{$\left | \eta \right | $}}
\newcommand{\dNdeta}       {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}\eta}}
\newcommand{\dNdy}         {\ensuremath{\mathrm{d}N/\mathrm{d}y}}
\newcommand{\dNdptdy}      {\ensuremath{\mathrm{d}N/{\rm d}\pt\mathrm{d}y}}
\newcommand{\dNdyst}       {\ensuremath{\sqrt{\frac{dN_\pi/dy}{s_T}}}}
\newcommand{\dNdetatr}     {\mathrm{d}N_\mathrm{tracklets}/\mathrm{d}\eta}
\newcommand{\dNdetar}[1]   {\mathrm{d}N_\mathrm{ch}/\mathrm{d}\eta\left.\right|_{|\eta|<#1}}
\newcommand{\lum}          {\, \mbox{${\rm cm}^{-2} {\rm s}^{-1}$}}
\newcommand{\barn}         {\, \mbox{${\rm barn}$}}
\newcommand{\m}            {\, \mbox{${\rm m}$}}
\newcommand{\ncls}         {\ensuremath{N_{cls}}}
\newcommand{\nsigma}       {\ensuremath{n\sigma}}
\newcommand{\dcaxy}        {\ensuremath{{\rm DCA}_{xy}}}
\newcommand{\dcaz}         {\ensuremath{{\rm DCA}_{z}}}
\newcommand{\EcrossB}      {E$\times$B}%{\ensuremath{{\rm E}\times{\rm B}}}
\newcommand{\bb}           {Bethe-Bloch}
\newcommand{\s}            {\ensuremath{\sqrt{s}}}

\newcommand{\hlab}         {\ensuremath{\eta_{\rm lab}}}
\newcommand{\ynn}         {\ensuremath{y_{\rm NN}}}
\newcommand{\ycms}         {\ensuremath{y_{\rm CMS}}}
\newcommand{\ylab}         {\ensuremath{y_{\rm lab}}}
\newcommand{\ppi}          {\ensuremath{{\rm p}/\pi}}
\newcommand{\kpi}          {\ensuremath{{\rm K}/\pi}}
\newcommand{\lpi}          {\ensuremath{{\rm \Lambda}/\pi}}
%\newcommand{\ppi}          {\ensuremath{(\pi^+ + \pi^-)/({\rm K}^+ + {\rm K}^-)}}
%\newcommand{\kpi}          {\ensuremath{({\rm p} + {\rm \bar p})/({\rm K}^+ + {\rm K}^-)}}
\newcommand{\mt}           {\ensuremath{m_{\rm T}}}
\newcommand{\snn}          {\ensuremath{\sqrt{s_{\rm NN}}}}
\newcommand{\snnbf}        {\ensuremath{\mathbf{{\sqrt{s_{\mathbf NN}}}}}}
\newcommand{\sonly}        {\ensuremath{\sqrt{s}}}
\newcommand{\Npart}        {\ensuremath{N_\mathrm{part}}}
\newcommand{\avNpart}      {\ensuremath{\langle N_\mathrm{part} \rangle}}
\newcommand{\avNpartdata}  {\ensuremath{\langle N_\mathrm{part}^{\rm data} \rangle}}
\newcommand{\Ncoll}        {\ensuremath{N_\mathrm{coll}}}
\newcommand{\Dnpart}       {\ensuremath{D\left(\Npart\right)}}
\newcommand{\DnpartExp}    {\ensuremath{D_{\rm exp}\left(\Npart\right)}}
\newcommand{\dNdetapt}     {\ensuremath{\dNdeta\,/\left(0.5\Npart\right)}}
\newcommand{\dNdetaptr}[1] {\ensuremath{\dNdetar{#1}\,/\left(0.5\Npart\right)}}
\newcommand{\dNdetape}     {\left(\ensuremath{\dNdeta\right)/\left(\avNpart/2\right)}}
\newcommand{\dNdetaper}[1] {\ensuremath{\dNdetar{#1}\,/\left(\avNpart/2\right)}}
\newcommand{\dndydpt}      {\ensuremath{{\rm d}^2N/({\rm d}y {\rm d}p_{\rm t})}}
\newcommand{\abs}[1]       {\ensuremath{\left|#1\right|}}
\newcommand{\signn}        {\ensuremath{\sigma^{\rm inel.}_{\rm NN}}}
\newcommand{\vz}           {\ensuremath{V_{z}}}
\newcommand{\Tfo}          {\ensuremath{{T}_{\rm kin}}}
\newcommand{\Tch}          {\ensuremath{{T}_{\rm ch}}}
\newcommand{\bT}           {\ensuremath{\beta_{\rm T}}}
\newcommand{\avbT}         {\ensuremath{\left< \beta_{\rm T}\right>}}
\newcommand{\avpT}         {\ensuremath{\left< \pt \right>}}
\newcommand{\muB}          {\ensuremath{\mu_{B}}}
\newcommand{\stat}         {({\it stat.})}
\newcommand{\syst}         {({\it sys.})}
\newcommand{\Fig}[1]       {Fig.~\ref{#1}}
\newcommand{\Figure}[1]    {Figure~\ref{#1}}
%\newcommand{\Ref}[1]       {Ref.~\cite{#1}}
%\newcommand{\green}[1]     {\textcolor{green}{#1}}
%\newcommand{\blue}[1]      {\textcolor{blue}{#1}}
%\newcommand{\red}[1]       {\textcolor{red}{#1}}
%\newcommand{\white}[1]     {\textcolor{white}{#1}}
\newcommand{\gevc}         {\ensuremath{{\rm GeV}/c}}
\newcommand{\mevc}         {\ensuremath{{\rm MeV}/c}}
\newcommand{\gs}           {\ensuremath{\gamma_{s}}}
\newcommand{\gq}           {\ensuremath{\gamma_{q}}}
\newcommand{\gc}           {\ensuremath{\gamma_{c}}}
\newcommand{\chindf}       {\ensuremath{\chi^{2}/{\rm NDF}}}
\newcommand{\avg}[1]       {\ensuremath{\left\langle#1\right\rangle}}
\newcommand{\etalab}       {\ensuremath{\eta_{{\rm lab}}}}
\newcommand {\gammas}			{\ensuremath{\gamma_{\mathrm{s}}}}
\newcommand{\DNDETAINEL}{5.31~$\pm$~0.18\xspace}
\newcommand{\DNDETAINELGTZERO}{6.46~$\pm$~0.19\xspace}
\newcommand{\DNDETAINELGTZEROONE}{6.61~$\pm$~0.20\xspace}
\newcommand{\inelgtzero}{INEL$>$0\xspace}
\newcommand{\average}[1]{\ensuremath{\langle #1 \rangle}\xspace}
\newcommand{\mpt}        {\ensuremath{\langle\pt\rangle}\xspace}
\newcommand{\nch}        {\ensuremath{N_\mathrm{ch}}\xspace}
\newcommand{\mnch}      {\ensuremath{\langle\nch\rangle}\xspace}
\newcommand{\nchacc}        {\ensuremath{N_\mathrm{ch}^\mathrm{acc}}\xspace}
\newcommand{\mnchacc}      {\ensuremath{\langle\nchacc\rangle}\xspace}
\newcommand{\inelg}     {\ensuremath{\mathrm{INEL}_{>0}}}



\newcommand{\dndeta}{\ensuremath{{\rm d}N_{\rm ch}/{\rm d}\eta}\xspace}
\newcommand{\dndpt}{\ensuremath{{\rm d}N_{\rm ch}/{\rm d}\pt}\xspace}
\newcommand{\etaless}[1]{\ensuremath{\left|\eta\right| < #1}\xspace}
\newcommand{\dndetaless}[1]{\ensuremath{{\rm d}N_{\rm ch}/{\rm d}\eta|_{\etaless{#1}}}\xspace}
\newcommand{\avdndeta}{\ensuremath{\langle \dndeta \rangle}}
\newcommand{\zvtx}{\ensuremath{z_\mathrm{vtx}}}


\newcommand{\pythiam}{\ensuremath{\mathrm{PYTHIA}\,8\,\mathrm{tune}}{\text -}4c}
\newcommand{\pythiashoving}{{\ensuremath{\mathrm{PYTHIA}\,8~\mathrm{String}~}}\ensuremath{\mathrm{Shoving}}}
\newcommand{\epos}{{\ensuremath{\mathrm{EPOS}\,~\mathrm{LHC}}}}
%\newcommand{\pythiashoving}{\ensuremath{\mathrm{PYTHIA}\,8~\mathrm{String}~}\linenomath{-}\ensuremath{\mathrm{Shoving}}}
\newcommand{\pttrig}{\ensuremath{p_\mathrm{T,\,trig}}}
\newcommand{\ptassoc}{\ensuremath{p_\mathrm{T,\,assoc}}}
\newcommand{\ptjet}{\ensuremath{p_\mathrm{T,\,Jet}}}
\newcommand{\ptlead}{\ensuremath{p_\mathrm{T,\,LP}}}
\newcommand{\pttrigassoc}{\ensuremath{p_\mathrm{T,\,trig\,(assoc)}}}









\renewcommand{\labelitemi} {$-$}
%==========================================================%
%%% inline warnings for internal discussion
%\newcommand{\warn}[1]      {\textbf{\textcolor{red}{[#1]}}}
\newcommand{\warn}[1]      {{\small\textbf{\textcolor{red}{(!\footnote{\textbf{(!)}~#1})}}}}
\newcommand{\warnin}[1]         {\textit{\textcolor{red}{(#1)}}}
%\newcommand{\warn}[1]      {#1}
%\newcommand{\warn}[1]      {{\small\textbf{(!\footnote{\textbf{(!)}~#1})}}\marginpar{\textbf{---}}}
\newcommand{\todo}[1]      {\textbf{\textcolor{red}{[TODO: #1]}}}
%%% fake numbers
\newcommand{\fake}[1]      {\textbf{\textcolor{red}{#1}}}
%\newcommand{\fake}[1]      {#1}
\newcommand{\final}[1]     {\textbf{\textcolor{blue}{#1}}}
\newcommand{\prelim}[1]    {\textbf{\textcolor{magenta}{#1}}}
\renewcommand{\mod}[1]       {\textbf{\textcolor{red}{#1}}}

